Integrals of motion from TBA and lattice-conformal dictionary

The integrals of motion of the tricritical Ising model are obtained by Thermodynamic Bethe Ansatz (TBA) equations derived from the A_4 integrable lattice model. They are compared with those given by the conformal field theory leading to a unique one-to-one lattice-conformal correspondence. They can also be followed along the renormalization group flows generated by the action of the boundary field \phi_{1,3} on conformal boundary conditions in close analogy to the usual TBA description of energies.

==> dati_I3_11cft.tex <==
I_3\text{ (CFT)}
0.0061979
4.2561979
19.131198
52.052045
22.560351
110.13688
55.125517
200.49775
112.78147
69.265146
35.980431


==> dati_I3_11tba.tex <==
    I_3\text{ (TBA)}
    0.0061979
    4.2561979
    19.131197
    52.052042
    22.560348
    110.13687
    55.125511
    200.49773
    112.78146
    69.265138
    35.980428


==> dati_I3_12cft.tex <==
I_3\text{ (CFT)}
-0.0063021
1.3686979
10.243698
33.732663
10.804733
78.939940
33.642011
16.699143
152.96762
78.030007
41.633949
43.143217


==> dati_I3_12cftexact.tex <==
I_3
-\frac{121}{19200}  
\frac{26279}{19200}
\frac{196679}{19200}
\frac{427559}{19200} + \frac{9{\sqrt{649}}}{20}
\frac{427559}{19200} - \frac{9{\sqrt{649}}}{20}
\frac{4309553}{134400} + \frac{216}{7( 16 - 7\alpha_i ) }
\frac{-16904148 + 3744000\kappa_i + 8284433\gamma_i}{19200(-12+7\gamma_i)}


==> dati_I3_12tba.tex <==
    I_3\text{ (TBA)}
   -0.0063020
    1.3686970
    10.243694
    33.732653
    10.804732
    78.939920
    33.642008
    16.699141
    152.96759
    78.029998
    41.633947
    43.143213


==> dati_I5_11cft.tex <==
I_5\text{ (CFT)}
-0.0028301
8.1731074
104.14545
556.20159
108.29650
1943.8246
551.34946
5280.2710
1919.0972
636.39114
209.28433


==> dati_I5_11tba.tex <==
    I_5\text{ (TBA)}
   -0.0028301
    8.1731074
    104.14545
    556.20155
    108.29648
    1943.8244
    551.34937
    5280.2705
    1919.0969
    636.39101
    209.28430


==> dati_I5_12cft.tex <==
I_5\text{ (CFT)}
0.0026543
1.3062480
37.203592
271.05745
34.613169
1117.9764
255.64791
64.926784
3367.1124
1071.0704
283.29346
365.24996


==> dati_I5_12cftexact.tex <==
I_5
\frac{1359}{512000}
\frac{668799}{512000}
\frac{19048239}{512000}
\frac{78251679}{512000} + \frac{297{\sqrt{649}}}{64}
\frac{78251679}{512000} - \frac{297{\sqrt{649}}}{64}
\frac{9(-864903608464-106010360777\alpha_i+173389286400{\alpha_i}^2)}{512000(-43504+17953\alpha_i)}
\frac{3( -2047389436 + 669441171\gamma_i+78848000{\gamma_i }^2+752339200\kappa_i+101068800\gamma_i \kappa_i  ) }{512000( -12 + 7\gamma_i  ) }


==> dati_I5_12tba.tex <==
    I_5\text{ (TBA)}
    0.0026543
    1.3062466
    37.203567
    271.05732
    34.613163
    1117.9759
    255.64786
    64.926773
    3367.1113
    1071.0702
    283.29343
    365.24990

